Efficient order picking methods in robotic mobile fulfillment systems

Robotic mobile fulfillment systems (RMFSs) are a new type of warehousing system, which has received more attention recently, due to increasing growth in the e-commerce sector. Instead of sending pickers to the inventory area to search for and pick the ordered items, robots carry shelves (called "pods") including ordered items from the inventory area to picking stations. In the picking stations, human pickers put ordered items into totes; then these items are transported by a conveyor to the packing stations. This type of warehousing system relieves the human pickers and improves the picking process. In this paper, we concentrate on decisions about the assignment of pods to stations and orders to stations to fulfill picking for each incoming customer's order. In previous research for an RMFS with multiple picking stations, these decisions are made sequentially. Instead, we present a new integrated model. To improve the system performance even more, we extend our model by splitting orders. This means parts of an order are allowed to be picked at different stations. To the best of the authors' knowledge, this is the first publication on split orders in an RMFS. We analyze different performance metrics, such as pile-on, pod-station visits, robot moving distance and order turn-over time. We compare the results of our models in different instances with the sequential method in our open-source simulation framework RAWSim-O.

==> sections/result_-_Kopie.tex <==
In this section, we first describe our open-source simulation framework with extensions and inputs for this paper in Section~\ref{subsec:framework}. After that, we show our simulation results in Section~\ref{subsec:results}. In Section~\ref{subsec:practical}, we show some practical points of view to the assumptions used in the simulation evaluations.
\subsection{Simulation framework} \label{subsec:framework}
We use in this paper RAWSim-O in \cite{RawSim.1}, an open-source agent-based and event-driven
simulation framework focusing at a detailed view of an RMFS. The source codes are available in \url{www.rawsim-o.de}. Figure~\ref{fig:mu_simulationframework} shows an overview of our simulation process, which is managed by the core \textit{simulator} instance. The tasks of the simulator contain:
\begin{itemize}
	\item Updating \textit{agents}, which can resemble real entities, such as robots and stations.
	\item Passing decisions to \textit{optimizer}, which can either decide immediately or buffer multiple requests and release the decision later. 
	\item Exposing information to a \textit{visualizer}, which allows optional visual feedback in 2D or 3D.
\end{itemize}

\begin{figure}[htb]
	\centering
	\includegraphics[width = 0.7\textwidth]{simulation-process-basic-light.pdf}
	\caption{Overview of the simulation process (see \cite{RawSim.1}).}
	\label{fig:mu_simulationframework}
\end{figure}



The hierarchy of all problems after new replenishment or pick orders' arrival in the system is illustrated in  Figure~\ref{fig:problemdependencies}. If a new replenishment order is received, the optimizers of ROA and RPS are responsible for choosing a replenishment station and a pod. This technically results in an insertion request, i.e. a request for a robot to bring the selected pod to the given workstation. If a new picking order is received, a new optimizer differed to \cite{RawSim.1}, called POA\&PPS, get the solution from our models and an extraction request for each item pick is generated. Note that, in \cite{RawSim.1} is first the POA optimizer called, after that, the PPS optimizer is called. Due to the introductions of split orders, parts of an order is allowed by the extraction requests to be assigned to different stations. Moreover, a pod is assigned to each extract request according to the result of the model. The item-capacity is counted by the extract requests at one station for each (part of) an order, which has at least one unfulfilled request at that station. Furthermore, the system generates store requests each time a pod is required to be transported to a storage location, and the PR optimizer decides the storage location for that pod. A number of these requests are then combined in an insertion task and assigned to a robot by a TA optimizer. All of the tasks result in trips, which are planned by a PP algorithm. 

\begin{figure}[H]
	\centering
	\includegraphics[width=0.85\textwidth]{problem-dependencies_integration.pdf}
	\caption{Order of decisions to be done triggered by receiving a pick or replenishment order}
	\label{fig:problemdependencies}
\end{figure}

The simulation framework conceptually consists of three different inputs: 
\begin{itemize}
	\item instance generator: generation of orders and further setting the system's surroundings (see Section~\ref{subsec:intance})
	\item layout configurator: determination of the characteristics and dimensions of the system layout (see Section~\ref{subsec:layout})
	\item optimizer configurator: specifying the decision rules for all operational problem in an RMFS (see Section~\ref{subsec:rules})
\end{itemize}
We describe these three input for our experiments in this paper in the following sections.
\subsubsection{Instance generation} \label{subsec:intance}
We generate three instance sets of 50, 150 and 250 orders. Each set include different number of SKUs, number of pods and SKUs per pod as listed in Table~\ref{tab:instance}. By considering all possible permutations, we have for each instance set eight instances. In total, we generate 24 instances. We test all methods in this paper with the pregenerated instances to see the efficienty of different models exactly. In a real RMFS, the orders are coming online. Our methods in this paper can be used in such case as well (see Section~\ref{subsec:practical}).

\begin{table}[H]
	\centering
	\begin{tabular}{ l l l }
		\hline
		Symbol & Description & Values\\
		\hline
		$|O|$ & Number of orders & 50, 150, 250 \\
		$|I|$ & Number of SKUs & 20, 100 \\
		$|P|$ & Number of pods & 50, 100 \\
		$\alpha$ & SKUs per pod & 2, 3 \\
		\hline
	\end{tabular}
	\captionof{table}{Instance parameters}
	\label{tab:instance}
\end{table}

First, the set of SKUs is generated as $I$ = \{$i_1$, ... , $i_{|I|}$\}. A shared storage strategy (as described in \cite{bartholdi.2017}) is applied to fill the pods. To determine the initial inventory of the pods, lists of all SKUs in randomized order are concatenated until the combined list includes at least $|P|$ $\cdot$ \ $\alpha$ elements. Then, for each pod $p_1, ..., p_{|P|}$, the inventory is determined by cutting off the first $\alpha $ items of the list.
For each order $o_1, ..., o_{|O|}$ the number of different SKUs in it is determined by a truncated (1 to $|I|$) geometric distribution with $p = 0.4$ (see Figure~\ref{fig:orderlen}). And the number of items of an SKU is set to 1. It is typical in online retailing that most of the orders contain very few line items, such as in \cite{bozer2018simulation} and \cite{onal2017modelling}. \todo{meaning?}The SKUs of the order are then chosen by sampling without replacement from $I$ using the probability mass function of a geometric distribution with $p = 5/|I|$, to account for the varying demand of different SKUs.

\begin{figure}[H]
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\captionsetup{justification=centering}
		\includegraphics[width=1\linewidth]{skusperorder.pdf}
		\captionof{figure}{Probabilities of order lengths for $|I|=20$}
		\label{fig:orderlen}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\captionsetup{justification=centering}
		\includegraphics[width=1\linewidth]{skuProbabilities.pdf}
		\captionof{figure}{Probabilities of SKUs for \\$|I|=20$}
		\label{fig:skus}
	\end{minipage}
\end{figure}

%\subsection{Simulation study} \label{subsec:simulation}



\subsubsection{Layout} \label{subsec:layout}
The layout is identical for all test instances and it is illustrated in Figure~\ref{fig:Layout}: 400 Pods, 504 storage locations in $2\times4$ blocks, 4 picking stations with a capacity of 15 items each and 8 robots. To see the effect of order picking better, we ignore the reflenishment process. Because the number of pods is higher than the values of $P$, empty pods can be neglected as they are not submitted to the model. %The number of robots is set to be large enough for our experiment as in \cite{Boysen.2017}, since we want to better see the effect of our performance metrics, such as pod-station-visits per order, robot distance per order, pile-on. 
The capacity of picking stations is similar to it used in \cite{Boysen.2017}. \cite{Boysen.2017} used a order-capacity of 6 orders. Since we use item-capacity instead of order-capacity, we Multiply 6 by 2.5, the mean of the distribution used to determine the number of SKUs per order (described in section \ref{subsec:intance}), leads to an item-capacity of 15. 
\vspace{0.5cm}
\begin{figure}[H]
	\centering
	\includegraphics[width=1\textwidth]{rawsim.png}
	\caption{Simulation layout \todo{Nils: update new figure, 8 robots}}
	\label{fig:Layout}
\end{figure}
\subsubsection{Decision rules} \label{subsec:rules}
Table \ref{tab:decrules} lists the decision rules for all operational problems in the evaluation. 

\begin{table}[H]
	\centering
	\begin{tabular}{ l l l  }
		\hline
		Decision Problem & Sequential & Integrated (without/with split orders)\\
		\hline
		POA & Pod-Match & Model \\
		PPS &  Demand & Model \\
		ROA &  not relevant & not relevant \\
		RPS &  not relevant & not relevant \\
		PR &  Nearest & Nearest \\
		PP & WHCA$^*_n$  & WHCA$^*_n$ \\
		\hline
	\end{tabular}
	\captionof{table}{Decision rules}
	\label{tab:decrules}
\end{table}
The decision rules selected for the sequential approach are based on \cite{RawSimDecisionRules}, since these combinations bring the best throughput.
There is a decision rule in \cite{RawSimDecisionRules} (called Common-Lines) and \cite{Wurman.2008} grouping similar orders at picking stations in POA. However, the decision rule Pod-Match in \cite{RawSimDecisionRules} for POA is appeared to perform better. This rule selects the pick order from the backlog that
matches best the pods already assigned to the station. The decision rule Demand for PPS choose the pod with
most units demanded in the backlog. 
The {\it ROA} and {\it RPS} problems concern on the replenishing process and thus are not relevant to our simulation tests, since we ignore the replenishment process.
The decision rule Nearest for {\it PR} assigns the closest parking space to each pod leaving the picking stations.
For the {\it PP} problem, non-volatile WHCA* in \cite{pathplanning} is used. And the Model for both POA and PPS is either the integrated model with or without split orders as described in Section~\ref{sec:model}.

\subsection{Simulation results} \label{subsec:results}
Each combination of method and instance is simulated ten repetitions to lessen the effect of randomness caused by other optimizers and simulation components. We use a cluster with twelve Intel Xeon X5650 Cores and 24 GB RAM to run the tests. The following performance metrics are tested:
\begin{itemize}
	\item the number of pod-station-visits per order
	\item the driven distance of robots per order
	\item pile-on: the average number of picks per visited pod
	\item throughput: the number of picks per hour
	\item turn-over time: measured from the time an order is open to the time the last item for that order is picked
\end{itemize}


Figure \ref{fig:podstationvisitsperorder} shows the average number of pod-station-visits per order relative to the sequential approach for each instance set of 50, 150 and 250 orders. Compared to the sequential approach for the number of pod-station-visits per order: The integrated model improves this performance by 20\% to 30\% for different instance sets, the split-among-station model (in short: split) improves about 50\%, and the split-over-time model (in short: timesplit) improves by 57\% to 80\%. 

%\begin{figure}[h]
%	\centering
%	\begin{subfigure}{0.45\textwidth}
%		\includegraphics[width = \textwidth]{relPSV_allOrder_8bots.pdf}
%		\caption{Pod-Station-visits per order}
%		\label{fig:podstationvisitsperorder}
%	\end{subfigure}
%	\begin{subfigure}{0.45\textwidth}
%		\includegraphics[width =\textwidth]{relDist_allOrder_8bots.pdf}
%		\caption{Robot distances per order}
%		\label{fig:distancesperorder}
%	\end{subfigure}
%\end{figure}
\begin{figure}[h]
	\centering
	\begin{minipage}{.45\textwidth}
		\centering
		\captionsetup{justification=centering}
		\includegraphics[width = \textwidth]{relPSV_allOrder_8bots.pdf}
		\captionof{figure}{Pod-station-visits per order}
		\label{fig:podstationvisitsperorder}
	\end{minipage}%
	\begin{minipage}{.45\textwidth}
		\centering
		\captionsetup{justification=centering}
		\includegraphics[width = \textwidth]{relDist_allOrder_8bots.pdf}
		\captionof{figure}{Robot distances per order}
		\label{fig:distancesperorder}
	\end{minipage}%
\end{figure}

Figure \ref{fig:distancesperorder} shows similar improvements for the average distances driven by robots to complete an order for each instance set. The correlation between pod-station-visits and distances driven by robots confirms our assumption in Section \ref{sec:intro}, that distances driven by robots can be reduced by minimizing the number of pod-station-visits. As our system layout shown in Figure \ref{fig:Layout} and the example of split orders shown in Figure~\ref{fig:example_splitting}, the distance between the inventory area and a picking station is in most cases greater than the distance between any two picking stations. Either a pod coming from the inventory area to a station or a pod coming from another picking station, it counts as a pod-station-visit. In the sequential approach, pods are often used between stations. However, all orders that
share same pod are assigned to a same station in the models. This can explain why distance per robot do not have exact same improvement as pod-station-visits per order.

 
Figure~\ref{fig:pileon} shows the pile-on \todo{more}. And it is not surprising that the solutions with more pile-on cause higher throughput as shown in Figure~\ref{fig:throughput}.

\begin{figure}[h]
	\centering
	\begin{minipage}{.45\textwidth}
		\centering
		\captionsetup{justification=centering}
		\includegraphics[width = \textwidth]{pileOn_allOrder_8bots.pdf}
		\captionof{figure}{Pile-on}
		\label{fig:pileon}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\captionsetup{justification=centering}
		\includegraphics[width = \textwidth]{throughput_allOrder_8bots.pdf}
		\captionof{figure}{Throughput, \todo{update figure, x-achsel missing}}
		\label{fig:throughput}
	\end{minipage}%
\end{figure}

In Figure~\ref{fig:comptime}, the average computational time of each iteration for each instance set is illustrated.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\textwidth]{comptime_allOrder_8bots.pdf}
	\caption{Computational time \todo{change the figure}}
	\label{fig:comptime}
\end{figure}


\subsubsection{Acceleration method} 
In the previous results, it is time-consuming to consider all orders in the backlog in the models, although it provide the best solutions. Therefore, we develop a heuristic to prefilter the orders and only a limit number of orderes is submitted to the model.
\todo{vorwahl algorithm}
\todo{Nils: Diagram trade-off quality and running time}
\todo{results of a large instance based on this vorwahl algorithm and limited number of orders is set to 10.}
%The backlog size for which a solution can be found without causing delays in the warehouse depends on a multitude of factors (such as the machine the solver is running on, the number of SKUs per order, number of pods containing each SKU) and can best be found by testing the respective instance with different backlog sizes.
%When the largest possible backlog size for which the model can be solved in an acceptable timeframe was found and the real backlog is larger than that, several criteria can be used for deciding which orders to submit. 


%Limiting the number of orders by handling them in batches of randomly chosen orders is equivalent to moving to a lower order count in Figure \ref{fig:podstationvisitsperorder} and Figure \ref{fig:distancesperorder}. When comparing the results of the model that allows splitting between stations and over time, reducing $|O|$ from 250 to 150 cuts the computing time in half (see Figure \ref{fig:comptime} and Table \ref{tab:comptime}) while the average distance driven to fulfill an order only increases by 10\% (see Figure \ref{fig:distancesperorder}).

%An even better solution than handling orders in batches could be to always submit a steady number of orders to the model in every iteration. When handling 250 orders in batches of 50, $t_1$ would have to be calculated 5 times. By always calling the model with $|O|$=50 until less than 50 orders are left, $t_1$ only has to be calculated once. As on average roughly twice the number of orders will be available to choose from in every iteration, the solution quality should be better compared to handling orders in batches. 

\subsection{Practical remarks} \label{subsec:practical}
We have some assumptions in Section~\ref{subsec:assumption}. Some of them might differ from the rea-world szenarios.
\begin{itemize}
	\item real-world orders: we use in this paper pregeneraated instances to see the performances of different approaches. Instead, in a real RMFS new orders would constantly come in while running the simulation and even completely new SKUs could be stocked. To account for this, our simulation RAWSim-O was recently extended by an interface to an ERP-System to allow for its use as a robot control system in real warehouses, as described in \cite{Xie.2018}. This new feature of the simulator could also be used in conjunction with the project presented in this paper, to implement the model presented here in a real warehouse and use real instances instead of pregenerated testing instances.
	\item capacity of packing stations: in the previous results we set the capacity of packing stations for split orders to be large enough to store all possible split orders if we can save the number of pod-station-visits. This capacity is differed from one company to another, therefore, it is possible that this capacity is small. In order to consider it, we can extend the models in Sections \ref{subsec:splitmodel} and \ref{subsec:timesplitmodel} with the following parameters, variables and constraints. We need two additional parameters: $C$ is the total capacities of packing stations (in other words: number of available split orders) and $N$ is number of stations. The binary variable $y_o^l$ is activiated if order $o \in O$ is splitted, while $n^l$ counts the number of actual split orders from the previous periods. Note that, this number is decreased by one if one split order is picked completely.
	\begin{align}
	& y_o^l \geq e_o/N, \; \forall o \in \mathcal{O}\label{eq:oap-40}\\
	& y_o^l \leq e_o, \; \forall o \in \mathcal{O}\label{eq:oap-41}\\
	& n^l+y_o^l \leq C, \; \label{eq:oap-42}\\
	& y_o^l \in \lbrace 0, 1 \rbrace, \; \forall o \in \mathcal{O} \label{eq:oap-43}
	\end{align}
	\todo{one experimental example}
	\item item-capacity: this capacity is used for comparing sequential and integrated approaches. The capacity of a picking station in real world is limited by the number of totes, which is depended on the size of an tote. There are following possibilities:
	\begin{itemize}
		\item using same size of totes as ususal, it might cause idle times in picking stations \todo{experimental example}
		\item using different sizes of totes, smaller ones for split orders to balance the capacity between orders and items
		\item using a separator in totes to balance the capacity between orders and items (an example: LocusBot in Figure~\ref{fig:locusBots})
	\end{itemize}
\begin{figure}[h]
	\centering
	\includegraphics[height=4.5cm]{locus_robot.jpg}
	\captionof{figure}{An example of using separators in totes}
	\label{fig:locusBots}
\end{figure}
	\item reliability of the simulation: as described in \cite{Xie.2018}, the simulation framework RAWSim-O is extended to connect an ERP-System and industry robots.
\end{itemize}
%\InlineComment{I think, we can use weighted items for capacity. From practical point of view there could be a difference between large items and small items. Formally the \eqref{eq:oap-5} can be written as
%	$\sum\limits_{o \in \mathcal{O}} \sum\limits_{i \in \mathcal{I}_o}w_{i} y_{i_oA} = C_A$.
%	For the non-split version it is sufficient to count the weights of the complete orders and use
%	order capacity. Something like $\sum\limits_{o \in \mathcal{O}}w^{\text{ord}}_{o} y_{oA} = C^{\text{ord}}_A.$
%}


